Semi-Supervised Multi-Task Learning Based Framework for Power System Security Assessment

This paper develops a novel machine learning-based framework using Semi-Supervised Multi-Task Learning (SS-MTL) for power system dynamic security assessment that is accurate, reliable, and aware of topological changes. The learning algorithm underlying the proposed framework integrates conditional masked encoders and employs multi-task learning for classification-aware feature representation, which improves the accuracy and scalability to larger systems. Additionally, this framework incorporates a confidence measure for its predictions, enhancing its reliability and interpretability. A topological similarity index has also been incorporated to add topological awareness to the framework. Various experiments on the IEEE 68-bus system were conducted to validate the proposed method, employing two distinct database generation techniques to generate the required data to train the machine learning algorithm. The results demonstrate that our algorithm outperforms existing state-of-the-art machine learning based techniques for security assessment in terms of accuracy and robustness. Finally, our work underscores the value of employing auto-encoders for security assessment, highlighting improvements in accuracy, reliability, and robustness. All datasets and codes used have been made publicly available to ensure reproducibility and transparency.

==> New_sections/2_Literature.tex <==
\section{Machine Learning in Power Systems Dynamic Security Assessment}

%Power system security assessment is a crucial process aimed at evaluating the ability of a power system to withstand disturbances and contingencies, e.g., short-circuit faults on the system’s components or outage events, without violating established operational limits \cite{fouad1988dynamic}. 
The nonlinear complex nature of dynamic security assessment has inspired researchers to develop advanced algorithms borrowed from well-established and mature domains for this task \cite{CREMER2021106571}. As a result,  machine learning algorithms for addressing this problem has shown remarkable strides over the years, moving from simpler models to more complex and powerful systems demonstrating remarkable capabilities in addressing various aspects of dynamic security. In this section, we provide a brief review of the evolution of ML-based solutions for power system dynamic security assessment.

Decision Trees (DT) were the first class of ML-based solutions to be proposed for security assessment, prominently used due to their high interpretability, which is crucial for establishing security rules for operators \cite{wehenkel1993decision, CREMER2021106571, wehenkel1998use}. Despite their advantages, DTs suffer from sensitivity to small changes in data and generally lag in performance compared to more advanced methods \cite{genc2010decision}. This drawback of DTs has been addressed in recent research which focused on using tree regularization to develop powerful models that are as accurate as neural networks while retaining the interpretability of the decision trees \cite{bugaje2021selecting, wu2018beyond}.

Neural Networks (NN) subsequently emerged as a powerful alternative, appreciated for their ability to model and predict complex dynamic behaviors like transient stability and voltage stability in power systems \cite{murzakhanov2020neural, xie2020review}. Although NNs significantly boost performance, both in static and dynamic security classification\cite{gholami2020static}, their lack of interpretability in addition to their unscalable performance on large power have been a major hurdle for widespread adoption in practice settings where understanding the decision-making process is essential \cite{zhang2019deep, wehenkel1997machine, zhang2021deep}.

To combine the benefits of multiple models, Ensemble Methods emerged, such as Random Forest (RF) and Gradient Boosting Machines (GBMs) were introduced. These methods leverage the strengths of numerous weak learners to form a more accurate and robust predictor \cite{zhukov2019ensemble}. Ensemble methods have shown enhanced performance in classifying transient stability and predicting post-contingency states in power systems\cite{zhukov2019ensemble, vakili2021machine}. However, like NNs, they generally do not provide the level of interpretability offered by simpler models like DTs, and they suffer from the curse of dimensionality, which in turn limits their application to large systems.

With the need for handling high-dimensional data and higher robustness to variations of inputs; Support Vector Machines (SVM) were adopted for their excellence in these areas \cite{dhandhia2020multi}. SVMs are particularly noted for their robustness against overfitting and hence missing data, a crucial feature for dynamic security assessment. Nevertheless, their performance diminishes with very large datasets, which poses a challenge for their application in larger power systems \cite{gomez2010support}.

The advances of deep learning brought varios neural network architectures such as Long Short-Term Memory (LSTM) networks and Graph Neural Networks (GNN). LSTM networks, effective in learning long-term dependencies, have been successful in modeling dynamic phenomena as time-series data, which has proven to be useful \cite{bush2021topological, ramirez2022convolutional, ren2021interpretable}. Moreover, GNNs, designed to handle graph-structured data, align naturally with the topology of power systems and have shown promising results in detecting cascading failures inlcuding security assessment \cite{zhou2021transient, ren2019fully}.

Also, Reinforcement Learning (RL) techniques have also been explored, particularly for their capability to facilitate real-time decision-making and control, which is pivotal for managing dynamic changes in power systems \cite{murzakhanov2020neural}. These methods learn optimal control policies that take into account a range of dynamic phenomena, providing a strategic edge in real-time operations \cite{liu2019reinforcement}.

Hybrid approaches have marked the latest development in this field, combining multiple machine learning techniques or integrating domain knowledge into learning algorithms to further enhance performance \cite{zhang2021confidence, lin2019reconstruction, liu2018accurate}. These hybrid models, which often blend deep learning with physics-based models or various learning algorithms, have demonstrated notable improvements in accuracy and robustness, paving the way for more reliable and efficient dynamic security assessments. Recent works in \cite{zhang2021deep, zhang2021confidence, zhang2019deep} incorporated the use of hybrid model through utilizing deep auto-encoders as feature representation layers to improve the scalability and robustness of the classifiers, and are currently achieving state-of-the-art results for power system security assessment.

In this paper, we introduce the Semi-Supervised Multi-Task-Learning (SS-MTL) framework, designed to refine the accuracy and precision of the classifier. Building on the evolution of techniques and features in the literature, we were motivated by the need for a more robust and scalable solution that could handle the complex and dynamic nature of power systems, while also incorporating topological awareness, and maintaining a degree of interpretability. The advancements in auto-encoders, particularly in their ability to create meaningful feature representations, inspired us to implement a modified auto-encoder in our framework. By optimizing the loss function and incorporating conditional masking \cite{zhang2021confidence}, we enhance the contingency awareness of the classifier, addressing a critical component of dynamic security assessment \cite{zhang2021confidence}, while modifying the loss function enables the network to learn feature representations more tailored to this application. Additionally, we employ a Feed-forward Neural Network (FFNN) as the classifier layer on top of the conditional auto-encoders, which demonstrates a notable reduction in missed alarms, outperforming traditional Bayesian classifiers \cite{zhang2021confidence}, Decision Trees (DT), and Support Vector Machines (SVM) \cite{genc2010decision, dhandhia2020multi}. To further improve the topological awareness of our framework—an essential aspect in accurately capturing power system dynamics—we propose a novel simple similarity model. This model utilizes Singular-Value-Sequence (SVS) \cite{bush2021topological} that was proven to capture power system attributes, achieving superior performance compared to existing techniques [citation]. This approach ensures a better understanding of the power system's topology, significantly enhancing the predictive capability of the security assessment framework. Finally, to provide a level of interpretability and certainty in the predictions, which is crucial for the operators, we incorporate the Mahalanobis distance \cite{mili1993robust} to estimate the uncertainty in the predictions generated from the FFNN based classifier.


==> New_sections/2_problem_formulation.tex <==
\section{Problem Definition}

Power system operators regularly perform security assessments to ensure the system can withstand potential disturbances. These assessments involve screening contingencies every 15 minutes and preparing contingency plans for critical scenarios. To do this, operators run both steady-state simulations (such as power flows to assess $N-1$ contingencies) and dynamic simulations \cite{hailu2023techniques}.
%
These simulations, however, pose significant challenges due to their complexity and computational demands. These simulations are generally NP-hard, involving systems of differential-algebraic equations with 10,000 degrees of freedom \cite{machowski1997power}. They require substantial computational power, memory, and often suffer from numerical instabilities and convergence issues. Additionally, checking for $N-k$ contingencies is a complex combinatorial problem \cite{sarkar2022search}. It is typically computationally infeasible to check even all $N-2$ contingencies in realistic systems with thousands of buses. Also, the safe operating region of a power system is a non-linear, non-convex space, making it infeasible to use analytical methods to determine it \cite{gunda2016analysis}.

Researchers have addressed these challenges by running extensive simulations to assess each operating point using approaches for efficient approximations to boost computation speed. They have developed several approaches to efficiently approximate solutions such as Transient Function Energy (TEF) methods \cite{pai1989energy}, thereby boosting computation speed. Also researchers have used stability certificates to extract sufficient conditions for sub-areas of the security region \cite{gholami2020fast}.
%
Recently, machine learning approaches have emerged as a promising alternative for addressing these challenges, particularly those related to speed and computational cost. Where, machine learning algorithms can be trained on large datasets and then used to infer results for new operating points or conditions, significantly enhancing the efficiency of security assessments.

A useful machine learning-based power system security assessment framework must possess the following characteristics:

\begin{itemize}
\item \textbf{High Coverage and Accuracy:} The framework should accurately classify the operating condition of a power system as secure or insecure for any new data point.
\item \textbf{High Sensitivity:} Since power system security assessment is a safety-critical application, missing an alarm can be very costly and potentially lead to undesired outcomes. Therefore, the framework must be exceptionally good at identifying insecure cases.
\item \textbf{Robustness:} The algorithm should be able to handle small changes in inputs that could lead to different system states. This includes detecting behaviors resulting from poor measurements or adversarial attacks.
\item \textbf{Interpretability:} Power system operators need to understand why the system is classified as secure or insecure. Hence, a level of interpretability is essential in the machine learning framework.
\item \textbf{Scalability:} Power systems can include thousands of buses, presenting a challenge to any algorithm's accuracy and efficiency. Additionally, power system topologies continuously change due to maintenance and other factors. The algorithm must be capable of withstanding these changes.
\end{itemize}

Generally, a machine learning algorithm requires a training dataset to infer and detect new points. Ideally, this dataset should consist of historical data and samples from the power system. However, historical data often lacks sufficient insecure operating points, which can hinder the algorithm's ability to detect such cases. Additionally, historical data might not cover all potential operating points of the power system, affecting the algorithm's performance on these points.

To train a reliable machine learning-based framework, we need to generate a comprehensive database that includes all potential cases with sufficient insecure instances to achieve high accuracy, coverage, and sensitivity. The techniques for generating this database are discussed further in \ref{generation}.

Throughout the development of the proposed framework in this paper, we have attempted to achieve all the above-mentioned characteristics.
